Articulated 3D Head Avatar Generation using Text-to-Image Diffusion Models

The ability to generate diverse 3D articulated head avatars is vital to a plethora of applications, including augmented reality, cinematography, and education. Recent work on text-guided 3D object generation has shown great promise in addressing these needs. These methods directly leverage pre-trained 2D text-to-image diffusion models to generate 3D-multi-view-consistent radiance fields of generic objects. However, due to the lack of geometry and texture priors, these methods have limited control over the generated 3D objects, making it difficult to operate inside a specific domain, e.g., human heads. In this work, we develop a new approach to text-guided 3D head avatar generation to address this limitation. Our framework directly operates on the geometry and texture of an articulable 3D morphable model (3DMM) of a head, and introduces novel optimization procedures to update the geometry and texture while keeping the 2D and 3D facial features aligned. The result is a 3D head avatar that is consistent with the text description and can be readily articulated using the deformation model of the 3DMM. We show that our diffusion-based articulated head avatars outperform state-of-the-art approaches for this task. The latter are typically based on CLIP, which is known to provide limited diversity of generation and accuracy for 3D object generation.

==> sections/supplement_implementation.tex <==
\subsection{Representation}
\paragraph{Shape.}
As described in the main text, the shape is implemented using the human head 3DMM FLAME~\cite{FLAME:SiggraphAsia2017} as a base mesh, and an MLP $\geonet_\theta$ modeling offsets from this mesh.
%
We use the modified FLAME model proposed in Neural Head Avatars~\cite{grassal2022neural}. This modified model uniformly subdivides the faces of the mesh (four-way subdivision), removes the faces belonging to the lower neck region, and adds additional faces close to the mouth cavity. This results in 16227 vertices on the FLAME model mesh rather than 5023.
%
Each vertex has an associated feature vector $c\in\R^d$. We set $d=32$ for all of our trained models.

The MLP $\geonet_\theta$ which models offsets takes in a concatenation of all the vertex positions of the neutral FLAME model $T\in\R^{16227\times3}$ and their associated vertex features $C\in\R^{16227\times d}$, and processes each one independently (16227 is the batch dimension), outputting vertex offsets $\in\R^{16227\times3}$. 
%
This MLP is implemented as a fully connected network with 3 hidden layers, each with hidden activation size 128. It uses $\relu$ as the activation function, with the final layer output being put through a $\tanh$ function and scaled by $10^{-1}$. This ensures that the offsets are not too large at initialization so that the mesh that is similar topologically to the FLAME template at initialization.

\paragraph{Texture.}
We model appearance as a feature texture map $\texture$ of resolution $512\times512\times4$, and use the UV coordinates defined with the FLAME model. The features of the texture map are defined in the latent space of Stable Diffusion v1.5~\cite{rombach2022high}, and thus each feature in the texture map is in $\R^4$. 
%
Rendered feature images from $\texture$ can be decoded into RGB space using the decoder in Stable Diffusion v1.5. This decoder also upsamples the feature images $8x$, resulting in $512\times512$ RGB images from a $64\times64$ feature image rendering. Note that these feature images can also be transformed into RGB images using the approximate linear transform from the latent space of Stable Diffusion v1.5 to RGB, as defined in~\cite{metzer2022latent}. However, we choose to use the provided decoder to upsample feature images in image space.

\subsection{Optimization}
\paragraph{Initialization.} 
We initialize the MLP $\geonet_\theta$ with the default ReLU MLP initialization, and initialize the per-vertex features $C$ in a zero-centered Gaussian distribution with $\sigma=0.02$.
%
Importantly, in initializing the vertex positions, we add a pre-computed set of offsets to the FLAME mesh in order to enlarge it. This extra offset is computed by applying Laplacian Smoothing~\cite{sorkine2004laplacian} with a negative strength, resulting in a smooth mesh with no intersections which is offset roughly along each vertex normal. We include a visualization of the expanded template mesh in Fig.~\ref{fig:mesh_supp}.
\begin{wrapfigure}{R}{0.45\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/meshes_supplement-c.pdf}
    \caption{\textbf{Enlarged template mesh initialization.} In order to provide a large enough canvas for the score distillation loss to paint a landmark-aligned texture onto, we enlarge the base FLAME template (left) with vertex offsets at initialization (right).}
	\label{fig:mesh_supp}
    \vspace{-1em}
\end{wrapfigure}
%
As described in the manuscript, this provides more area for the texture-only optimization to paint texture on, which can then be trimmed by subsequent geometry optimization steps.
%
For example, the enlarged mesh gives room for the texture-only optimization to paint head accessories on, which can then be converted into consistent geometry via the segmentation loss. This is apparent in the examples shown in the main paper where the enlarged scalp results in the ability to paint on head and hat details to be consistent with a specific prompt.

\paragraph{Score distillation loss.}
We use the score distillation loss implementation provided in Score Jacobian Chaining~\cite{wang2022score}. Unlike DreamFusion~\cite{poole2022dreamfusion}, which uses the Imagen~\cite{saharia2022photorealistic} diffusion model, the Stable Diffusion v1.5 model directly predicts denoised images directly instead of the predicting the noise to subtract from a noised image. In practice, this implementation results in similar performance.
%
Note that this loss function never provides a direct value for text-image similarity, but instead the diffusion model is used to compute gradients with respect to a value which represents this. We do not scale or alter these gradients by any value.

Like in other works using score distillation as a loss function, we find it necessary to use a high classifier-free guidance in order to obtain converged results~\cite{poole2022dreamfusion, wang2022score}. We use a classifier-free guidance parameter of 100. As classifier-free guidance is known to produce oversaturated and non-realistic images in generation, we hypothesize that this is the reason for some of the oversaturation and cartoonish effects on some of our generated 3D head avatars.

\paragraph{Texture only optimization and shading cues.}
For texture optimization, we use a learning rate of $8\times10^{-3}$. We perform 6,000 iterations of texture-only optimization to start the optimization process, and then 2,000 more iterations after every 4,000 iterations of geometry and texture optimization.
%
In this step, we use only the score distillation loss, and backpropagate from rendered images into the texture $\texture$ only. Since gradients propagated into the geometry ($\beta, \theta, C$) are likely noisy, we manually ensure that appearance gradients are not propagated here.

As described in the main text, to encourage semantic features to be generated in the correct locations (i.e. mouth on the FLAME model mouth), the rendered textured images are blended with textureless renders of the offset mesh.
%
These are obtained as in Eq. 5, and the amount of influence from the textureless image is controlled by $\alpha$. We tune this parameter over the course of training as follows: for the first 4,000 iterations, $\alpha = \frac{\texttt{curriter}}{4000}$, i.e. linearly increasing to $1$. After this, we set $\alpha$ to be uniformly distributed between $0.6$ and $1.0$, leading to more contribution from the rendered feature image on average. This schedule encourages the texture to align features with the correct landmarks early in optimization, so that the score distillation gets caught in a local minimum with features aligned. Then, later in optimization, lower $\alpha$ allows the texture to focus on more detailed appearance features without accounting for the contribution from the textureless image, which is not used in rendering final images or videos.

\paragraph{Geometry optimization.}
Following the texture-only optimization step, we perform a joint geometry and texture optimization step. In this case, we use a learning rate of $8\times10^{-3}$ for texture parameters $\texture$, and a learning rate of $1\times10^{-4}$ for geometry paramters $\beta$, $\theta$, $C$. We propagate gradients from the score distillation loss only into $\texture$, as in the texture-only optimization step. However, we propagate gradients from the segmentation loss $\loss{seg}$ and regularization loss $\loss{geom}$ into the parameters modeling geometry: $\beta$, $\theta$, $C$.

After every 2,000 iterations of geometry optimization, we compute a look-up table of approximate segmentation masks for views which can be observed during training. For this, we set the expression and pose parameters to be in the neutral position, and vary the viewpoint direction, computing a separate segmentation mask for each elevation and azimuth $e,a$ which can be sampled at training with $1^\circ$ granularity. In our results, we do not vary $e$, and sample $a\in[-30^\circ,30^\circ]$, resulting in us computing 61 segmentation masks for each $1^\circ$ interval in $[-30^\circ,30^\circ]$. 
%
We compute these segmentation masks using the Segment Anything~\cite{kirillov2023segany} model. This model returns various segmentation masks at different levels of specificity (i.e., it can segment only hat or hair). We take the segmentation mask which has the largest amount of pixels, and includes pixels known to intersect with the center of the FLAME template. This way, we are able to obtain a segmentation mask of the entire head, including accessories, and use it as supervision in $\loss{seg}$.

We compute $\loss{seg}$ using the stored segmentation masks (updated every 2,000 iterations) and upsampled, rasterized soft masks at each iteration, as described in Eq. 6 of the main paper. We multiply this loss by a factor $\lambda=1000$.

\paragraph{Geometry regularization.} We apply $\loss{geom}$ as described in Eq. 7. We use the following parameters for weighting the relative regularization terms: $\lambda_1=0.5$, $\lambda_2=5000$, $\lambda_3=5000$. We implement $\loss{off}$ by computing offsets from the base FLAME mesh at a specific expression, rather than the expanded FLAME mesh used at initialization. We compute $\loss{lap}$ using PyTorch3D~\cite{ravi2020pytorch3d} mesh Laplacian smoothing, where the Laplacian is computed with uniform weights. Finally, we compute $\loss{prior}$ by computing a weighted L2 difference with the mesh Laplacian of the ground truth FLAME model mesh (without any enlargement). 
%
We weight the parts of the mesh in computing this Laplacian difference in the following way: all regions are weighted equally with weight $1$, but the "scalp" region is weighted $10^{-1}$, the "face" region is weighted $5\times10^{-1}$, and the "forehead" region is weighted $5\times10^{-1}$. This is because these regions have the most area for accessories or complex geometry on the head, and thus should not align as closely with the FLAME template.

\paragraph{Viewpoint and pose sampling.}
As we focus on articulation of the facial expression, we sample viewpoints facing the front of the FLAME model with 0 elevation and azimuth in $[-30^\circ, 30^\circ]$. All camera positions are taken at a radius of $0.7$ from the origin, where the FLAME template is centered. This allows the views to focus on the front of the face, and not worry about using text prompt conditioning to accurately fit the back of the head and prevent multiple faces from appearing~\cite{poole2022dreamfusion}.
%
We randomly vary poses during training. We sample these poses from a dataset obtained by running the tracking on the first sample video provided in the NHA~\cite{grassal2022neural} repository. This corresponds to 1496 different expressions used during training. We use the tracking from the second provided as video as validation expression parameters to drive our generated models. 

During training, in order to improve the quality of the generated results, we pre-pend ``a photo of the face of'' to each of the generated prompts. % Beyond this, we need more advanced text-based conditioning in order to get proper generated textures.

\paragraph{Rasterization.}
As described in the text, we use a differentiable mesh rasterizer based on SoftRasterizer~\cite{liu2019soft} in Pytorch3D~\cite{ravi2020pytorch3d} to rasterize images and text. 
%
For rasterizing feature images to be passed into the score distillation loss, we perform a "hard" rasterization which does not blur mesh faces and softly blend overlapping rasterized feature values. This results in gradients only being passed into $\texture$, and a hard silhouette mask which does not pass gradients into $\beta,\theta,C$. We also use this setting to rasterize the textureless shading guidance mesh image.
%
When rasterizing soft masks to be used in geometry optimization, we use rasterizer parameters $\sigma=10^{-4}$, $\gamma=10^{-4}$, and 75 faces per pixel. This ensures that the rasterization of the mask is differentiable with respect to the vertex positions. Note that when optimizing both texture and geometry, we must perform two rasterizations - one with hard blending and one with the differentiable soft blending.

Since the rasterization of features is performed at the low resolution of $64\times64$, there can be faces which are never observed in training pose variation, resulting in uncanny visualization when the heads are animated into new expressions after optimization. Thus, we rasterize feature images at a resolution of $512\times512$, and bilinearly downsample them into $64\times64$ resolution before passing them into the decoder to be again upsampled. This downsampling and blurring in rendered features encourages gradients to be passed into all features located in the texture, as the higher resolution rasterization does not suffer from aliasing. Since the blurring is done in feature-space, it does not result in as blurry of a resulting image after being decoded.
%
Additionally, to prevent the model from painting the background into $\texture$, we vary the background at each training iteration between a randomly sampled uniform color and a checkerboard with two randomly sampled colors and boxes of a randomly sampled size between 15 and 25 pixels.

\paragraph{Computational Complexity.} 
We train each model using an NVIDIA RTX6000 GPU. Each model consumes approximately 12GB of VRAM and trains for approximately 1.5 hours, corresponding to 20,000 iterations. We used a total of 4 RTX6000 GPUs in training models and preparing results for the paper.

\subsection{Rendering videos.} 
When rendering videos, we are able to drive the optimized avatar representation using new FLAME expression and pose parameters. We retain the geometry by keeping the parameters $\beta,\theta,C$ which were optimized for during training.
%
As the decoder performs an $8x$ up-sampling operation, converting $64\times64$ feature images to $512\times512$ RGB images, unwanted flickering artifacts can be visible as small changes in the feature value are propagated into a larger region of the image. Thus, we rasterize features at $512\times512$ resolution, and bi-linearly downsample these feature images to $64\times64$ before decoding them into $512\times512$ images.

\subsection{Evaluation}
We evaluate using the CLIP-R Precision metric proposed in Dream Fields~\cite{jain2022zero}. We similarly evaluate this metric using three different CLIP models, on both rendered RGB images and rendered textureless offset mesh images.
%
We compute the recall metric using 100 rendered images for each target prompt. Each of these images are rendered with randomly selected FLAME expression and pose parameters from the training dataset, and randomly selected views where azimuth  $a\in[-30^\circ,30^\circ]$. We add random noise as the background (instead of having a uniform color) to prevent the CLIP model from focusing exclusively on the silhouette of the head and biasing the results to head-related prompts. We do the same for the rendered textureless images of the mesh in order to measure geometric consistency with the prompts.

We evaluate CLIP-R Precision for 7 prompts. These prompts are: ``an alien'', ``Elon Musk'', ``a zombie'', ``a sumo wrestler'', ``a construction worker'', ``a graduate student'', ``a man with a large afro''. We pre-pend the modifier ``a photo of the face of'' to each of these prompts. As potential false positives, we include 267 randomly scraped prompts from the DreamFusion gallery. However, these prompts come from a very different distribution than the list of head prompts which we use, and thus CLIP obtains almost perfect recall by just focusing on the fact that each image is a head. Thus, we add an additional 60 prompts, many of which were used to generate results for our method. Each of these prompts is also pre-pended with ``a photo of the face of.''
%
The list of prompts is here: "a man with a large afro", "a man wearing a wearing a top hat", "a man wearing a hat", "a wizard wearing a hat", "a man with large spiky hair", "a zombie", "an alien", "Batman", "Keanu Reeves", "Rihanna", "Shaq", "Jackie Chan", "a senior citizen", "a doctor", "a graduate student", "a sumo wrestler", "a construction worker", "Leonardo DiCaprio", "Cristiano Ronaldo", "Ryan Gosling", "Margot Robbie", "Elon Musk", "Dwayne Johnson", "Shrek", "a lawyer", "a teenager", "a gardener", "a pilot", "a firefighter", "a soldier", "a scientist", "a police officer", "a Jedi", "Godzilla", "James Bond", "Bill Gates", "Lionel Messi", "LeBron James", "Roger Federer", "an astronaut", "a man with a large chin", "a man wearing a baseball hat", "a female scientist", "Santa Claus", "Hulk", "an anime character", "Cloud Strife", "a man with a swollen face", "Jeff Bezos", "Mark Zuckerberg".

\paragraph{Baselines.}
As described in the main text, we compare to the baselines of Text2Mesh~\cite{michel2022text2mesh} and ClipFace~\cite{aneja2022clipface}. Both of these are capable of converting text prompts into 3D representations (and with some modifications, head avatars). These methods both use CLIP. Details of their implementation and evaluation is included in the following two paragraphs. 

\paragraph{Text2Mesh.} We use the official Text2Mesh repository, and make a few edits to ensure that the representation is able to create a 3D Head Avatar comparable to ours. Specifically, we use the same FLAME model from NHA and our method (with the expanded number of vertices) as the base mesh on which Text2Mesh operates. Additionally, we modify the training scheme to sample viewpoint and FLAME expression and pose parameters to exactly match the training of our method. We keep other training details, such as the loss formulation with CLIP and rendered image augmentations, the same as the default Text2Mesh.
\begin{figure}[t!]
\centering
	\includegraphics[width=\textwidth]{figures/ClipFace_supplement-c.pdf}
	\caption{\textbf{Additional ClipFace results.} We show results from ClipFace for prompts shown in the main paper with different initial latent codes in the validation set. Additionally, we show two different prompts: ``a graduate student'' and ``an alien''. The different latent codes change the generated identity slightly for each given prompt.
    }
	\label{fig:clipface_supp}
\end{figure}

\paragraph{ClipFace.} We obtained an implementation of ClipFace from the authors along with a pre-trained GAN model, which we used directly for prompt-specific optimization and evaluation. We additionally obtained training and validation latent codes (each representing a different identity in the ClipFace GAN) from the authors for training the mapping network for a specific prompt. This mapping network was then trained for each specific prompt in the 7 previously mentioned prompts we use for evaluation. We train each of the mapping networks using the default hyperparameters (and FLAME model) for 25,704 iterations, at which point the validation samples appeared to resemble the specific text prompt.
%
For rendering images, we select a random latent code (representing a random latent identity) in the validation set. This identity is then transformed to be compatible with the text prompt by passing it through the trained mapping network for that prompt. We use default values for evaluating this network, and sample the initialization latent codes from the provided validation dataset by the authors.

==> sections/supplement_results.tex <==
For additional results of our method, such as rendered videos demonstrating articulation and multi-view rendering, please see our website at:

\vspace{.4em}
\centerline{
\texttt{\href{https://www.computationalimaging.org/publications/articulated-diffusion/}{computationalimaging.org/publications/articulated-diffusion/}}
}

\paragraph{ClipFace.}
In Fig.~\ref{fig:clipface_supp}, we include additional results from ClipFace. These results show more examples for various evaluation prompts with different latent vectors used as initial input, corresponding to different person identities in the ClipFace GAN. We can see that using different initial latent codes makes minor differences in the output generated result, but the results remain consistent with the prompt. 
%
However, all of the generated results still suffer from the same types of artifacts in ClipFace - lack of flexibility in the prior to model diverse, humanoid subjects, and lack of geometry optimization, as the result is constrained to generating the texture on the FLAME mesh. We note that ClipFace provides other functionality, such as text-driven expression generation. This is an orthogonal contribution to ours, as we use the text to only generate appearance and shape for an avatar for which expression can be controlled.

\paragraph{Text2Mesh.}
\begin{figure}[t!]
\centering
	\includegraphics[width=\textwidth]{figures/Text2Mesh_supplement-c.pdf}
	\caption{\textbf{Additional Text2Mesh results.} We show additional results from Text2Mesh on different evaluation prompts. As with the prompts shown in the main paper, Text2Mesh tends to produce results which appear to contain textures resembling the prompt but are not globally cohesive, such as in the ``alien'' example. For some prompts, such as ``a man with a large afro'', the lack of geometric regularization results in divergence.
    }
	\label{fig:ttm_supp}
\end{figure}
We include additional Text2Mesh results in Fig.~\ref{fig:ttm_supp}. Similar to the results in the main paper, Text2Mesh produces textures resembling the prompt but are not globally cohesive. This is because in order to get CLIP supervision on 3D representations to converge, methods like Text2Mesh require rendering multiple cropped and augmented images at every training iteration. This is well studied as a method used in order to avoid local minima in the CLIP latent space~\cite{lee2022understanding}. Additionally, the lack of geometric regularization results in unstable training for some prompts, as is visible in Fig.~\ref{fig:ttm_supp}. The textures resemble the final prompt, but do not generate cohesive nor high-quality results.
\begin{figure}[t!]
\centering
	\includegraphics[width=\textwidth]{figures/SJC_supplement-c.pdf}
	\caption{\textbf{Score Jacobian Chaining results.} We show results generated by generic text-to-3D methods such as Score Jacobian Chaining, which also uses the Stable Diffusion v1.5 model. These results generated are not controllable or compatible with a 3DMM like FLAME. We note that despite text conditioning the result to generate a face, the method still generates a full upper body. Our method generates results which are qualitatively similar in quality, but are guaranteed to be articulable 3D head avatars.
    }
	\label{fig:sjc_supp}
\end{figure}

\paragraph{Score Jacobian Chaining.}
We emphasize that while methods like DreamFusion~\cite{poole2022dreamfusion} and Score Jacobian Chaining~\cite{wang2022score} are able to convert text prompts into 3D representations, they are \textbf{not} compatible with 3D head avatar generation. This is because these methods fundamentally have no control over what is generated besides the prompt. For example, in Fig.~\ref{fig:sjc_supp}, we generate results for the prompts ``a man wearing a tophat'' and ``Drake'' using the same prompt pre-conditioning, i.e. "a photo of the face of". While these methods are able to produce a 3D representation, this representation is not aligned with a 3DMM such as FLAME and doing so is not a trivial task. We emphasize that our method produces 3D results which are qualitatively on-par with these methods, but retain the ability to control what is generated: an articulable 3D head avatar. 

\paragraph{Different diffusion models.}
We emphasize that our formulation is not dependent on the specific diffusion model used, i.e. Stable Diffusion v1.5. Other diffusion models can be used in the score distillation loss formulation, often producing better results. For example, the recently released DeepFloyd-IF~\cite{deepfloyd} has led to significant improvements in open source, non-articulated text-to-3D projects~\cite{stable-dreamfusion}, including significantly reducing the saturation of generated results. This is a fruitful direction of future work in generating higher quality 3D head avatars from text.
